Preliminary Study on Incremental Learning for Large Language Model-based Recommender Systems

Adapting Large Language Models for Recommendation (LLM4Rec) has shown promising results. However, the challenges of deploying LLM4Rec in real-world scenarios remain largely unexplored. In particular, recommender models need incremental adaptation to evolving user preferences, while the suitability of traditional incremental learning methods within LLM4Rec remains ambiguous due to the unique characteristics of Large Language Models (LLMs). In this study, we empirically evaluate two commonly employed incremental learning strategies (full retraining and fine-tuning) for LLM4Rec. Surprisingly, neither approach shows significant improvements in the performance of LLM4Rec. Instead of dismissing the role of incremental learning, we attribute the lack of anticipated performance enhancement to a mismatch between the LLM4Rec architecture and incremental learning: LLM4Rec employs a single adaptation module for learning recommendations, limiting its ability to simultaneously capture long-term and short-term user preferences in the incremental learning context. To test this speculation, we introduce a Long- and Short-term Adaptation-aware Tuning (LSAT) framework for incremental learning in LLM4Rec. Unlike the single adaptation module approach, LSAT utilizes two distinct adaptation modules to independently learn long-term and short-term user preferences. Empirical results verify that LSAT enhances performance, thereby validating our speculation. We release our code at: https://github.com/TianhaoShi2001/LSAT.

==> 5_related_backup.tex <==
\section{RELATED WORKS}

\subsection{LLM-based Recommendation}
% 1.研究中利用LLM进行推荐的范式可以根据其 generally categorized according to the roles they serve in the recommendation pipeline： \ie, feature engineering, feature encoder, scoring/ranking functions.
% 2. Feature engineering 的方法利用LLM为传统推荐模型从原始的文本信息中提取额外的文本特征。 
% 3. feature encoder的方法中LLM作为辅助文本特征提取器来丰富用户/item表征。
% 4. Nevertheless, this method still relies on traditional models making it difficult to take advantage of the generative ability of LLMs.
% 5.对于利用LLM4Rec作为scoring/ranking functions. 一种做法是用in-context learning使 LLM学会 learn the recommendation task through autoregression using appropriate instructions and examples. However, this method is often limited due to the size constraints of LLM inputs and the lack of recommendation knowledge [3, 30]. 
% [30] Is chatgpt a good recommender? a preliminary study.
% 6.为了克服这一限制，一些方法例如 TALLRec [3], Bigrec, employs recommendation data in an instruction-tuning phase to improve the recommendation capability of the LLM.
% 我们的研究主要关注使用推荐数据进行微调，并把LLM作为 scoring/ranking functions的范式，研究在实际推荐场景下，incremental learning对这些模型的影响。
The application of Large Language Models in recommender systems can be broadly classified based on their distinct roles in the recommendation pipeline: feature engineering~\cite{borisov2022language,carranza2023privacy}, feature encoding~\cite{he2022ptm4tag,yuan2023go}, and scoring/ranking functions~\cite{tallrec,bigrec}. Feature engineering~\cite{borisov2022language,carranza2023privacy} entails employing LLMs to extract additional textual features from raw textual data, integrating them into traditional recommender models. Within feature encoding~\cite{he2022ptm4tag,yuan2023go}, LLMs serve as auxiliary text feature extractors to enhance the representation of users and items. However, it is worth noting that both these approaches still rely on traditional models, limiting the exploitation of LLMs' generative capabilities. 

For scoring/ranking functions~\cite{wang2023zero,chen2023palr,tallrec,bigrec}, a viable approach involves leveraging in-context learning, which enables the LLM to acquire proficiency in the recommendation task through autoregression~\cite{wang2023zero,chen2023palr}. These methods require providing the LLM with appropriate instructions and examples for guided learning. It's essential to recognize that this approach faces limitations due to the restricted input size of LLMs and the scarcity of recommendation-specific knowledge~\cite{liu2023chatgpt, tallrec}. 
To overcome these limitations, researchers have introduced techniques like TALLRec~\cite{tallrec} and BIGRec~\cite{bigrec}, which include an instruction-tuning phase integrating recommendation data to enhance LLMs' recommendation capabilities using the LoRA technique. 
Specifically, our research investigates the impact of incremental learning on the last category of LLM4Rec.
% , providing valuable insights for their practical deployment.


% Specifically, our research focuses on the impact of incremental learning on LLM4Rec.
% Our research focuses on adapting LLMs for recommendation
% utilizing recommendation data to refine LLMs as the fundamental framework for scoring and ranking functions. 
% Specifically, we investigate the impact of incremental learning for LLM4Rec
% Specifically, we investigate the impact of incremental learning on these models in real-world recommendation scenarios.


% 不用的部分：Researchers in the field primarily investigate LLM-based recommendations from two perspectives
% 第一种方法是是在零样本训练的情况下，使用in-context learning使 LLM学会 learn the recommendation task through autoregression using appropriate instructions and examples. However, this method is often limited due to the size constraints of LLM inputs and the lack of recommendation knowledge [3, 30]. 为了克服这一限制，一些方法考虑使用推荐数据对LLM进行微调，提高其推荐性能。其中一些方法利用LLM作为feature encoder，然后使传统推荐模型利用提取的embedding或是特征
% The first approach involves in-context learning (ICL), where LLMs like ChatGPT learn the recommendation task through autoregression using appropriate instructions and examples. However, this method is often limited due to the size constraints of LLM inputs and the lack of recommendation knowledge [3, 30].
% The second approach involves fine-tuning LLMs on recommendation data, as LLMs lack relevant recommendation data in their pre-training phase [3, 28]. One method uses the LLM to obtain item embeddings, which are then fed into traditional recommendation models (e.g., SASRec [23]). However, this method still relies on traditional models and limits the ability to leverage the generative capabilities of LLMs.
% Two existing studies, TALLRec [3] and InstructRec [55], employ recommendation data in an instruction-tuning phase to improve the recommendation capability of the LLM. However, their evaluation is limited to the CTR scenario or conducted through negative sampling and does not explore the LLM's ability to rank all items.




\subsection{Incremental Learning in Recommendation}

% P1讲推荐系统更新重要的相关工作
% 1.在推荐系统中，新的物品持续出现，且用户和item偏好持续变化，这使得在推荐系统中更新很有必要
% 例： in the recommendation systems, new items always emerge on an hourly to daily basis [6], and item preferences of users continuously change [7], Practical recommender systems need to retrain periodically
% 2.已经有不少工作研究了及时的数据更新对传统推荐模型的影响，前两个例子里选两个简单写一下。例如：faster model updates and synchronization are shown to have positive effects on online model performances. For example, in Ekko [1], an large-scale distributed recommender system showed that faster model synchronization leads slight gain in online model performances. On the other hand, In [2], faster model training and shorter update period via collisionless embedding table verified better model performances.
% [3] quantitatively demonstrate the delayed model update actually harms the model performance by increasing the number of cold users and cold items increase and decreasing overall model performance. 
% 3.这些方法都强调了在推荐系统中模型更新的重要性，但至今没有研究探索更新对LLM4Rec的影响，我们是第一个定量地研究它的工作。

% [1] EKKO：A large Scale deep learning recommender system with Low-Latency model update
% [2] Monolith:Real time recommendation system with collisionless embedding table
% [3] How Important is Periodic Model Update in Recommender Systems?
In the recommender systems, the continual emergence of new items~\cite{landia2022recsys} and persistent shifts in user preferences~\cite{zheng2018drn} necessitate frequent updates to maintain system effectiveness. Extensive studies have scrutinized the impact of timely data updates on traditional recommendation models. For instance, Ekko~\cite{sima2022ekko}, a large-scale distributed recommender system, demonstrated a modest improvement in online model performances through faster model synchronization. Additionally, 
% research such as~\cite{liu2022monolith} showcased enhanced model performances with faster training and shorter update periods using a collisionless embedding table. 
quantitative experiments~\cite{updateImportant} underscored that delayed model updates detrimentally affect performance by increasing cold users and items, leading to an overall decline in model efficacy. 
Previous investigations underscore the vital role of incremental learning in recommender systems. However, there is a gap in exploring this aspect in LLM4Rec. Our study investigates the unexplored issues of incremental learning for LLM4Rec.
% While these investigations highlight the crucial role of incremental learning in recommender systems, no prior research has explored it on LLM4Rec. Our study uniquely investigates the unexplored incremental learning on LLM4Rec.

% P2
% 1.There are some works of model retraining in recommender systems. 
% 2.参考SML文章的introduction第二段以及related works 1. fine-tuning, which updates the model based on the new interactions only [35, 41]. 它非常高效，但可能面临模型遗忘的问题 2. full retraining 采样全部的样本并更新模型，它虽然准确率高，但训练代价大 3. sample-based retraining: sampling a faction of historical interactions and mixing them with new interactions for model updating. 
% 3.此外，还有一类文章利用meta-learning 进行模型更新，在保持长期偏好的同时促使模型可以快速迁移到新数据上，例如SML，它采用meta-learning 用新数据更新模型并设计transfer net to converts the old model, achieve a good trade-off between long-term and short-term modeling by optimizing for the future performance；
% 4.我们的研究中，采用最具代表性的fine-tuning和full retraining研究incremental learning对LLM4Rec的影响。
Various methods have been proposed for model retraining in recommender systems. (1) Fine-tuning~\cite{rendle2008online,wang2018neural}: This involves updating the model based solely on new interactions, offering efficiency but facing the challenge of potential model forgetting. (2) Full retraining: This approach entails sampling the entire dataset for model updating, achieving high accuracy at the cost of considerable training resources. (3) Sample-based retraining~\cite{diaz2012real,wang2018streaming}: Selectively sampling a portion of historical interactions and integrating them with new interactions constitutes this method. (4) Meta-learning-based methods~\cite{sml,longshort}: This approach strives to preserve long-term preferences while facilitating rapid adaptation to new data with meta-learning. 
% Illustrated by SML~\cite{sml}, meta-learning is employed to update the model with fresh data. SML further introduces a transfer net to transform the existing model, achieving a balance between long-term and short-term modeling, optimizing for future performance. 
In our research, we empirically investigate the impact of incremental learning on LLM4Rec by employing two representative techniques: fine-tuning and full retraining. 
Furthermore, we introduced an approach leveraging distinct LoRA modules to concurrently capture long-term and short-term preferences, offering insights for the incremental learning of LLM4Rec from the perspective of the capacity of the LoRA module.


% 5.这句我最后来加:此外,我们提出了xxproposal。
% 废弃：例如LSTTM，它designs a temporal MAML to accelerate model adaptation to users’ short-term preferences.make full use of both internal and external information to leverage user short-term and long-term preferences, finding an industrial balance between effectiveness and efficiency in practice.

==> 9_ethical_consideration.tex <==
% \section*{Ethical Consideration}

% % 推荐重要，伦理重要
% % 本文数据集两个用的合规
% % 第二本文研究推荐公平，公平性时可信ai重要组成部分。当然，公平并不是可信的全部，接下从与可信ai密切相关的其他两个维度谈论本文章可能的伦理问题
% % 1.透明度，本技术涉及对用户的敏感属性收集以及重建，根据xxxx整个过程都需要用户知情并同意才可以进行，收集的敏感属性也只能用于特定目的，而不是利用它单纯追求推荐性能优化推荐系统，这可能造成更大的歧视，这需要法律法规完善与有效监管。
% % 2.隐私保护。因为本文的研究收集敏感属性，并且对缺失敏感属性进行重建，这可能带来隐私泄露的风险。从伦理角度，可信的AI必须保护这些隐私数据。从企业角度，需要对这些隐私信息利用差分隐私，联邦学习等方法进行保护。对于用户，用户应该拥有拒绝提交或是重建敏感属性的权力，对于已经提交或是重建的敏感属性，用户也应该拥有遗忘敏感属性的权利。
% % recommender systems have a wider impact on users and on society more broadly，例如 它影响着人们获取的信息，并影响着人们的偏好。因此，推荐系统中的伦理问题应该被严肃地对待。
% % Recommender systems wield a profound influence over both individual users and the broader societal landscape. They exert their impact by shaping the information individuals are exposed to and molding their preferences. Consequently, the ethical considerations within recommender systems should be seriously discussed.
% % First, we utilize publicly available MovieLens and Tenrec data in a purely
% % observational and non-intrusive manner. We follow all ethical
% % regulations set by GroupLens Research and Tencent Inc.
% % Second, 本文关注的公平性是可信推荐系统的重要概念之一，提升公平性可以有效提升推荐系统的可信程度。当然，公平并非可信推荐系统的唯一指标，接下来我们将从以下两个与可信推荐系统有关的概念谈谈本文可能涉及的伦理问题。
% % Recommender systems exert a far-reaching impact on both individual users and the broader societal fabric. They exert their influence by shaping the information to which individuals are exposed and by molding their preferences accordingly. As such, the ethical dimensions inherent to recommender systems necessitate rigorous scrutiny.
% % In our research endeavor, we conscientiously adopt a stance of employing publicly accessible MovieLens and Tenrec data through a wholly non-invasive observational approach. Throughout our investigative process, we remain steadfast in adhering to the ethical regulations meticulously stipulated by the eminent GroupLens Research as well as the esteemed Tencent Inc.
% % Moreover, a central tenet of our study revolves around the crucial concept of fairness within the realm of credible recommender systems. The enhancement of fairness holds the potential to significantly bolster the overall credibility of these systems. It is important, however, to underscore that fairness is but one facet among multiple indicators of a credible recommender system. In the subsequent discourse, we delve into two interconnected concepts closely related to credible recommender systems, expounding on the ethical quandaries that our paper may potentially navigate.
% % Recommender systems exert a broad impact on individual users and society, providing personalized information filtering based on user interests and preferences.
% Recommender systems significantly impact both users and society by delivering personalized information filtering based on user interests and preferences.
% As such, the ethical aspects of recommender systems require serious discussion~\cite{ethical-rec}. 
% Our research centers on improving recommendation fairness despite limited sensitive attributes, enhancing the trustworthiness of the recommender system.
% % In our research, we focus on improving recommendation fairness with limited sensitive attributes, enhancing the trustworthiness of the recommender system. 
% Nevertheless, additional ethical concerns persist. Below, we discuss the potential ethical issues of our DROFLSA in line with two ethical criteria for trustworthy recommender systems. 
% % 然而，仍然存在一些其他的伦理担忧，下面我们从两个与可信推荐系统相关的伦理标准谈论本技术可能的伦理问题
% % Nevertheless, fairness is just one aspect of trustworthy recommender systems. In the following, we delve into interconnected concepts and the potential ethical consideration our paper may navigate.

% \noindent\textbf{Transparency.}
% Transparency is a critical principle of trustworthiness, which requires that the appropriate information should reach the relevant parties~\cite{diaz2023connecting}.
% % As this study encompasses the collection and reconstruction of sensitive user attributes, according to legal frameworks such as the GDPR, the entire process mandates user awareness and explicit consent as prerequisites.
% % Our study delves into the collection and reconstruction of sensitive user attributes.
% % As this study encompasses the collection and reconstruction of sensitive user attributes, 
% In line with achieving transparency, we underscore the importance of comprehensively apprising users about the purpose of utilizing sensitive attributes and obtaining explicit consent before the collection and reconstruction of such confidential information of our method. Otherwise, a non-transparent collection process of sensitive attributes can lead to user distrust and result in legal compliance issues.
% % we emphasize the necessity of ensuring users are fully informed of the purpose of utilizing sensitive attributes and provide explicit consent before the collection and reconstruction of sensitive attributes to improve fairness.
% % Furthermore, it's essential to align the utilization of sensitive attributes with user consent. Otherwise, blindly utilizing sensitive attributes to enhance recommendation accuracy could worsen fairness, thereby harming the system's trustworthiness.

% % Furthermore, it's crucial to tightly regulate the acquisition of sensitive attributes with the goal of promoting fairness.
% % The procurement of sensitive attributes is exclusively earmarked for the enhancement of fairness, as expounded within this study, refraining from their utilization as mere features in pursuit of optimizing recommender system performance. The heedless pursuit of this alternative path could potentially amplify discriminatory effects, thus underscoring the necessity for comprehensive legal refinement and effective regulatory oversight.

% \noindent\textbf{Privacy.} 
%  A trustworthy recommender system must safeguard private data~\cite{diaz2023connecting}. As our proposed method involves the collection of sensitive attributes and the reconstruction of missing sensitive attributes, there are potential risks of privacy leakage. 
% To address this concern, it is necessary for enterprises to protect this private information, employing techniques like differential privacy~\cite{abadi2016deep} and federated learning~\cite{rodriguez2020federated}. Regarding users, the right to refuse the submission or reconstruction of sensitive attributes should be ensured. Additionally, for sensitive attributes that have already been submitted or reconstructed, users should also have the right to request the forgetting of such attributes.
% % The collection of sensitive attributes and subsequent reconstruction of missing sensitive attributes entail potential risks of privacy infringement. From an enterprise perspective, it becomes imperative to safeguard these privacy-sensitive data through techniques such as differential privacy and federated learning. As for users, they should possess the prerogative to decline the submission or reconstruction of sensitive attributes. Moreover, for those sensitive attributes already submitted or reconstructed, users should also possess the right to invoke the principle of attribute forgetfulness.
% % 本研究涉及对用户的敏感属性收集以及重建，根据一些法律如GDPR规定整个过程都需要用户知情并同意才可以进行。收集的敏感属性也只能用于特定目的，而不是利用它单纯追求推荐性能优化推荐系统，这可能造成更大的歧视，这需要法律法规完善与有效监管。

% % employ publicly accessible MovieLens and Tenrec data non-invasively, following GroupLens Research and Tencent's ethical guidelines. Moreover, this study 


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

